Efficient Recovery Learning using Model Predictive Meta-Reasoning

Operating under real world conditions is challenging due to the possibility of a wide range of failures induced by execution errors and state uncertainty. In relatively benign settings, such failures can be overcome by retrying or executing one of a small number of hand-engineered recovery strategies. By contrast, contact-rich sequential manipulation tasks, like opening doors and assembling furniture, are not amenable to exhaustive hand-engineering. To address this issue, we present a general approach for robustifying manipulation strategies in a sample-efficient manner. Our approach incrementally improves robustness by first discovering the failure modes of the current strategy via exploration in simulation and then learning additional recovery skills to handle these failures. To ensure efficient learning, we propose an online algorithm called Meta-Reasoning for Skill Learning (MetaReSkill) that monitors the progress of all recovery policies during training and allocates training resources to recoveries that are likely to improve the task performance the most. We use our approach to learn recovery skills for door-opening and evaluate them both in simulation and on a real robot with little fine-tuning. Compared to open-loop execution, our experiments show that even a limited amount of recovery learning improves task success substantially from 71% to 92.4% in simulation and from 75% to 90% on a real robot.

==> includes/6_limitations.tex <==
While the full problem is a POMDP, we solve it approximately using pessimistic failure discovery and optimistic recovery learning.
This results in a mis-match between the discovered and actual failures leading to sub-optimal prioritization of recovery learning. 
Second, we discover failures purely in simulation which precludes many failures that are not modeled by the simulator.
% Third, we do not currently report evfa our approach on a real robot.
Finally, our allocation algorithm Value-MAB is myopic and may find sub-optimal allocations.
We will address some of these limitations in our future work.
In particular, (1) we are conducting more thorough evaluation of our approach and (2) we are interested in using a realistic state estimator to discover failures and learn recoveries in the belief space.
% (1) The discovered distribution of failures may not match the true distribution which depends on the state estimation being used.
% (2) Since we discover failures purely in simulation, we may miss failures due to unmodeled variations in the task.
% There is a lot of variety in tasks in the real world which may not always be feasible to simulate due to limited information of capabilities of the simulator.
% This suggests that actively discovering failures by acting in the real environment is crucial for robustness.

